Learning, fast and slow

Animals can learn efficiently from a single experience and change their future behavior in response. However, in other instances, animals learn very slowly, requiring thousands of experiences. Here I survey tasks involving fast and slow learning and consider some hypotheses for what differentiates the underlying neural mechanisms. It has been proposed that fast learning relies on neural representations that favor efficient Hebbian modification of synapses. These efficient representations may be encoded in the genome, resulting in a repertoire of fast learning that differs across species. Alternatively, the required neural representations may be acquired from experience through a slow process of unsupervised learning from the environment.

==> sections/Annotations.tex <==
\section{Annotated Literature}

Hick 1952: An early and influential paper on human reaction time vs task difficulty. Measures the difficulty by the mutual information between stimulus and response.

Amir 2020: A recent example of the information-theoretic approach to the complexity of behavior using a control model to predict the animal's actions.

Kandel 2014 \citep{kandelMolecularSystemsBiology2014}: A wide-ranging review of learning mechanisms. Starts from a psychological perspective on different forms of memory, and eventually turns to mechanisms at the cellular and molecular level.

Citri 2008 \citep{citriSynapticPlasticityMultiple2008}: Good review of mechanisms of synaptic plasticity. Includes homosynaptic, heterosynaptic, and homeostatic mechanisms.



==> sections/Discussion.tex <==
\section{Discussion}
TBD, here are some potential topics:

\subsection{Do animals in the real world ever benefit from slow learning?}
\begin{outline}
\1 Species with a short lifetime cannot invest 10000 attempts into learning a single bit action. This applies to the laboratory mouse. It reaches sexual maturity in less time than it takes to learn a 2AFC task in the lab. 
\1 Songbird: two kinds of learning
 \2 memorizing template fro the father's song: this can be quite fast, ~10 repeats.
 \2 practicing song to emulate the template and perfect its reproducible structure, takes longer, ~1000 repeats?
 \2 But note this is a mating signal. Like the peacock’s feathers it signals that this individual can waste resources for a perfectly pointless display. In this case the finch signals that it spent lots of time practicing that it didn't need to spend foraging or hiding from predators.
\1 Human artists, musicians, athletes, etc. Those talents require 1000s of days of training. 
 \2 We admire these people precisely because what they do is so unnatural.
 \2 Again, these activities can be seen as mating displays.
 \2 Presumably learning is so slow because there is not a pre-existing neural representation matched to those tasks, e.g. for the finger movements needed to play Bach's Cello Suites.
 \2 Perhaps the neocortex offers the hardware for slow learning of an efficient neural representations. More useful for animals that live long enough so this actually matters. Bigger cortex offers more opportunities for parallel representations. Empirical correlation between longevity and number of cortical neurons: https://pubmed.ncbi.nlm.nih.gov/30350858/
\end{outline}

\subsection{Constraints on biological learning}

\begin{outline}
\1 Have we just been missing a more powerful mechanism of synaptic learning that allows a much wider range of network variables to influence any given synapse?
 \2 This seems unlikely, because the information must get to that synapse within the time scale of the sensory-motor events that are to be associated, 0.1-1 s.
 \2 One mode for signaling at that speed is electrical conduction. But there are only two neurons connected to the synapse electrically: the pre- and the post-synaptic neuron.
 \2 Another mode is chemical diffusion, but only with restricted range: 0.1 s corresponds to 10 um. That is the typical distance between synapses, so diffuse release (e.g. "spillover") could play a role, but only from one or a few other synapses.
\end{outline}


==> sections/Measures_Of_Learning_old.tex <==

\section{Quantitative measures of learning} \label{sec:info-methods}
We are considering a general task defined by a set of states $s_i$ and actions $a_j$ that lead from one state to another. For example, in a simple 2-alternative-forced-choice task to teach a rodent odor classification, the states are given by the two stimuli $s_1 = $ "odor A" and $s_2 = $ "odor B". The actions consist of turning to one of the two reward ports to lick a drop of water: $a_1 = $ "lick left" and $a_2 = $ "lick right". The rodent's task is to learn that $s_1$ should be followed by $a_1$ and $s_2$ by $a_2$. Typically the training regimen involves rewards and punishments that follow correct or incorrect choices of actions. This framework generalizes very broadly to any task that can be described by a graph with states as the nodes, actions as the edges, and rewards distributed along the graph. This includes many natural behaviors like navigation towards a target, and cognitive tasks like games.

\begin{figure}
  \centering
    \includegraphics[width=0.5\linewidth]{figures/Task_Graphs.pdf}
    \caption{\textbf{Graphs that define behavioral tasks.} \textbf{(a)} A typical 2-alternative-forced-choice task, with states defined by stimuli $s_1$ and $s_2$ and actions of the animal $a_1$ and $a_2$. The square states terminate a trial with reward (green) or no reward (red). \textbf{(b)} A more complex task in which the animal starts in state $s_1$ and then navigates a binary tree by turning left ($a_1$) or right ($a_2$) or backing up to the previous state ($a_0$). Only one of the end points of the tree is rewarded. The task can be implemented as navigation in a binary maze.
    }
\label{fig:task-graphs}
\end{figure}

\subsection{How complex is the task?}
Because learning involves the extraction of information from experience, it seems natural to apply information-theoretic tools to measure learning. For example, a useful measure of task complexity is the mutual information between states and actions under the rules that the task represents. If $p(s,a)$ is the joint probability of states and actions under the task rules, then the mutual information is

\begin{equation}
T = \textrm{Task complexity} = \sum_{s,a} p(s,a) \log_2 \frac {p(s,a)}{p(s)p(a)}
\label{eqn:task-complexity}
\end{equation}

where $p(s)$ and $p(a)$ are the probabilities of state $s$ and action $a$ respectively.
In the above example of 2AFC odor classification, the two odors appear at equal frequency, so $p(s_1)=p(s_2)=0.5$ and similarly for the two actions $p(a_1)=p(a_2)=0.5$. The task rules demand that $p(s_1,a_1)=p(s_2,a_2)=0.5$ and $p(s_1,a_2)=p(s_2,a_1)=0$. This can all be summarized in a contingency table (Table \ref{tab:2AFC-table}a). From Eqn \ref{eqn:task-complexity} the complexity of this task is 1 bit. Another way to see this is that the state completely specifies which of the two actions should be taken, and that requires 1 bit of information.

If the two states (e.g. odor stimuli) are used at unequal frequency, the task becomes less complex. For example if odor A appears 90\% of the time (Table \ref{tab:2AFC-table}b), the complexity is only 0.47 bits. This results because much of the time the correct action can be chosen even by guessing.

The formalism also extends to tasks that are specified probabilistically. For example the stimulus may indicate which of the two response ports is more likely to be baited with a reward [cite experiments like this] (Table \ref{tab:2AFC-table}c). 

\begin{table}[]
\centering
\begin{tabular}{cl|cc|}
\bf{a} &                        & \multicolumn{2}{c|}{$a$}       \\
\multicolumn{1}{l}{}    &                        & \multicolumn{1}{c|}{L}   & R   \\ \hline
\multirow{2}{*}{$s$}    & \multicolumn{1}{c|}{A} & \multicolumn{1}{c|}{0.5} & 0   \\ \cline{2-4} 
                        & \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{0}   & 0.5 \\ \hline
\end{tabular}
\quad
\begin{tabular}{cl|cc|}
\bf{b} &                        & \multicolumn{2}{c|}{$a$}       \\
\multicolumn{1}{l}{}    &                        & \multicolumn{1}{c|}{L}   & R   \\ \hline
\multirow{2}{*}{$s$}    & \multicolumn{1}{c|}{A} & \multicolumn{1}{c|}{0.9} & 0   \\ \cline{2-4} 
                        & \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{0}   & 0.1 \\ \hline
\end{tabular}
\quad
\begin{tabular}{cl|cc|}
\bf{c} &                        & \multicolumn{2}{c|}{$a$}       \\
\multicolumn{1}{l}{}    &                        & \multicolumn{1}{c|}{L}   & R   \\ \hline
\multirow{2}{*}{$s$}    & \multicolumn{1}{c|}{A} & \multicolumn{1}{c|}{0.4} & 0.1   \\ \cline{2-4} 
                        & \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{0.1}   & 0.4 \\ \hline
\end{tabular}
\vspace{3mm}
\caption{
\label{tab:2AFC-table}
\textbf{Contingency tables for a 2AFC task.} The joint probability $p(s,a)$ of states ($s=$ "A" or "B") and actions ($a=$ "L" or "R"). 
{\bf{(a)}} Equal use of the two stimuli. $I=1$ bit. 
{\bf{(b)}} Unequal stimulus use: "A" occurs 90\% of the time. $I=0.47$ bit.
{\bf{(c)}} Stochastic rule: the stimulus determines which of the two actions is more likely correct. $I=0.28$ bit.
}
\end{table}

The approach also extends to cases with many more options. For example a typical "Animal menagerie" book for children has 26 pictures of animals, one for every letter of the alphabet. When the parent asks "where's the kangaroo?" that amounts to a 26-alternative-forced-choice task. The task complexity is $\log_2 26 = 4.7 \, \rm{bits}$. Every time the child learns to pair a new word correctly with the picture, it acquires $\frac{1}{26} \log_2 26 = 0.18 \, \rm{bits}$.

\subsection{How much did the animal learn?}
By comparing the animal's actions before and after training we can evaluate how much it changed its behavior. Suppose the joint distribution of states and actions is $q(s,a)$ prior to learning and $r(s,a)$ after learning. The difference between $q$ and $r$ reflects how much the behavior has changed. A natural measure of this is the so-called KL-distance between the two distributions \citep{coverElementsInformationTheory2012}.

\begin{equation}
C = \textrm{Change in behavior} = D_{\textrm{KL}}(r,q)
= \sum_{s,a} r(s,a) \log_2 \frac {r(s,a)}{q(s,a)}
\label{eqn:task-learned}
\end{equation}

In the above example of a 2AFC task, suppose the animal's performance after training saturates at 85\% correct actions. Then it has learned only $C=0.39$ bits. An animal that performs at 70\% correct~\citep{guoFlowCorticalActivity2014} has learned only 0.12 of the possible 1.0 bits.

This measure serves also if the action distribution is essentially continuous. For example in a study on motor learning in rats~\citep{kawaiMotorCortexRequired2015}, animals were trained to produce two taps exactly 700 ms apart. Before training the animals produced tapping intervals of 400 ± 200 ms (mean ± SD). After training the distribution was 700 ± 170 ms. If the two distributions were roughly Gaussian, the KL-distance amounts to 0.55 bits. This is how much the rat learned about the task it was trained to do. 

\subsection{How well does the animal perform?}
The change in behavior measured by Eqn \ref{eqn:task-learned} does not specify the direction of that change. The animal may have altered its responses in ways that are unrelated to the stimuli, or even opposed to the intended goal of training. For example, in a 2AFC task, the measure $C$ is the same if the animal associates stimuli and actions in the opposite order. This may well result from poor design of the training regimen. Thus one also wants to know how close the animal's behavior is to that specified by the task rules. Again, one can use the KL-distance, this time between the actual behavior after training and that intended by the task rules:

\begin{equation}
E = \textrm{Error}  = D_{\textrm{KL}}(r,p)
= \sum_{s,a} r(s,a) \log_2 \frac {r(s,a)}{p(s,a)}
\label{eqn:task-error}
\end{equation}

This is a measure of errors the animal makes relative to the intended "perfect" behavior. Thus one obtains a measure of performance by subtracting the errors from the task complexity:

\begin{equation}
P = \textrm{Performance}
= T-E 
\label{eqn:task-performance}
\end{equation}

Because $E$ is guaranteed non-negative, the task complexity represents an upper bound on performance in the task.

For example, this measure of animal behavior has been used to assess learning in song birds~\citep{metsAutomatedApproachQuantitation2018}. Here the target behavior is the tutor bird's song, characterized by an action distribution $p(a)$. The tutee's song, similarly characterized by $r(a)$, differs from the target, and the error is measured by the KL-distance. Alternatively, one can take a more model-based approach and formalize the animal's actions as the output of a control system ~\citep{amirValuecomplexityTradeoffExplains2020}. In this framework, learning alters the parameters of the control system. Again, one can measure the amount that was learned by the KL-distance between the distribution of parameters before and after training.

\subsection{Why use information theory?}
What recommends these information-theoretic measures of behavior, as compared to any other statistical tool that correlates states with actions? An important desirable for any measure of task complexity is additivity: If a task is composed of two independent subtasks, the complexity of the combined task should be the sum of the individual complexities. One can show that the mutual information of Eqn \ref{eqn:task-complexity} satisfies this additivity constraint. For example, this allows us to derive the complexity of the binary decision tree in Figure \ref{fig:task-graphs}b: The shortest route from state $s_1$ to the reward requires one correct 2-way decision followed by two correct 3-way decisions. If the actions "left", "right" and "back" are equally probable to begin with, the complexity is $T = \log_2{2} + 2 \times \log_2{3} = 4.2$ bits. A larger tree with 64 end nodes, as used in a recent experimental study~\citep{rosenbergMiceLabyrinthExhibit2021}, will have task complexity $T = \log_2{2} + 5 \times \log_2{3} = 8.9$ bits.

% A second argument is that the mathematical statements of information theory offer some useful relationships if one adopts this formalism. For example, one can show that a binary reinforcer (reward vs no reward) can teach the animal at most 1 bit about the rules of the task, thus setting a limit to the learning rate, namely how fast the performance $P$ can improve over successive trials.


